On the Performance Prediction of BLAS-based Tensor Contractions

Tensor operations are surging as the computational building blocks for a variety of scientific simulations and the development of high-performance kernels for such operations is known to be a challenging task. While for operations on one- and two-dimensional tensors there exist standardized interfaces and highly-optimized libraries (BLAS), for higher dimensional tensors neither standards nor highly-tuned implementations exist yet. In this paper, we consider contractions between two tensors of arbitrary dimensionality and take on the challenge of generating high-performance implementations by resorting to sequences of BLAS kernels. The approach consists in breaking the contraction down into operations that only involve matrices or vectors. Since in general there are many alternative ways of decomposing a contraction, we are able to methodically derive a large family of algorithms. The main contribution of this paper is a systematic methodology to accurately identify the fastest algorithms in the bunch, without executing them. The goal is instead accomplished with the help of a set of cache-aware micro-benchmarks for the underlying BLAS kernels. The predictions we construct from such benchmarks allow us to reliably single out the best-performing algorithms in a tiny fraction of the time taken by the direct execution of the algorithms.

==> Makefile <==
PDFLATEX = pdflatex -shell-escape -recorder

TARGET = main.pdf

TEXFILES = *.tex figures/*.tex

default: once

once: 
	$(PDFLATEX) main

twice:
	make once
	make once

figs:
	time make -j 4 -f main.makefile

ffigs:
	time make -j 4 -f main.makefile -B

bib:
	bibtex main

all:
	make once
	make figs
	make bib
	make once
	make ffigs
	make twice

bg:
	make once < /dev/null 2>&1 1> /dev/null &

check: $(TEXFILES)
	for file in $(TEXFILES); \
	do \
		aspell --lang=EN --mode=tex check $$file; \
	done

clean:
	rm -rf main.{blg,fls,aux,log,toc,pdf,lof,out,figlist,makefile,pyg} figures/externalized/*


==> future.tex <==
The prediction framework presented in this paper is designed for general
loop-based algorithms that encapsulate their computation in compute-kernels.
\pdj{ok, but as opposed to what?}
The algorithms for tensor contractions analyzed in this paper are 
prominent representatives of such a class. 
However, in practice various extensions to other
problems and solution algorithms are possible.
\pdj{don't get this last sentence.}
\begin{itemize}
\item New libraries, such as BLIS \cite{blis}, provide BLAS-like
    compute-kernels with a more flexible interface, in terms of which tensor
    contractions can be cast without the need for copy operations.
  \pdj{so what?}
\item Contractions involving three or more tensors or sequences of
  contractions play an important role in practice. 
  In such cases, our methodology could
  be applied to find the optimal contraction-ordering or loop-fusing
  algorithms.
  \pdj{Wut?}
\item Due to the contiguous data layout assumed for all the tensors,
  in certain contractions 
  it would be possible to combine indices of the same type 
  (free or contracted) and treat the result as a single dimension with respect
  to BLAS invocations.
  For instance, in $C_{abc} = A_{ai} B_{ibc}$, the free indices $b$ and
  $c$ appear always (in $B$ and $C$) together and in the same order;
  \pdj{we can't say ``hence'' yet. We also need them to be ``adjacent'' (consecutive)}
  hence, it would be possible to treat them as a single index $d = bc$, 
  reducing the entire contraction to $C_{ad} = A_{ai} B_{id}$ --- i.e., a single \gemm.
\end{itemize}
\pdj{what of we had tensors with leading dimensions?  (i.e., tensor being a
  sub-tensor of laregr one)}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

